The Generative AI Ethics Playbook

The Generative AI Ethics Playbook provides guidance for identifying and mitigating risks of machine learning systems across various domains, including natural language processing, computer vision, and generative AI. This playbook aims to assist practitioners in diagnosing potential harms that may arise during the design, development, and deployment of datasets and models. It offers concrete strategies and resources for mitigating these risks, to help minimize negative impacts on users and society. Drawing on current best practices in both research and ethical considerations, this playbook aims to serve as a comprehensive resource for AI/ML practitioners. The intended audience of this playbook includes machine learning researchers, engineers, and practitioners who are involved in the creation and implementation of generative and multimodal models (e.g., text-to-text, image-to-image, text-to-image, text-to-video). Specifically, we provide transparency/documentation checklists, topics of interest, common questions, examples of harms through case studies, and resources and strategies to mitigate harms throughout the Generative AI lifecycle. This playbook was made collaboratively over the course of 16 months through extensive literature review of over 100 resources and peer-reviewed articles, as well as through an initial group brainstorming session with 18 interdisciplinary AI ethics experts from industry and academia, and with additional feedback from 8 experts (5 of whom were in the initial brainstorming session). We note that while this playbook provides examples, discussion, and harm mitigation strategies, research in this area is ongoing. Our playbook aims to be a practically useful survey, taking a high-level view rather than aiming for covering the entire existing body of research.

==> stage-template.tex <==
\section{\textbf{Stage \#X}}

\stageHeader{STAGE NAME}
\mysubtitle{SUBTITLE}

Intro Text Here

\mysubtitle{Topics of Interest}\\
\emph{You can click on the topics below to jump to their sections.}
\begin{itemize}
    \item \textcolor{blue}{\hyperref[sec:add_hyperref_here]{Topic Name}}
    \item \textcolor{blue}{\hyperref[sec:add_hyperref_here]{Topic Name}}
\end{itemize}
\todo{Make sure to add hyperlinks to those sections here}
% \newpage

\subsection{Transparency \& Documentation Checklist}

In this stage of the AI lifecycle, we recommend that you discuss and document the following:
\begin{itemize}
    \item[$\square$] Add action items here
    \item[$\square$] Add action items here
\end{itemize}
\newpage

% TOPIC OF INTEREST SUBSECTION (CAN COPY PASTE THIS BOILERPLATE BELOW)

\subsection{Name of Topic of Interest}
\label{sec:add_section_label_here}
\underline{\textbf{Definitions / Relevant Terms}}\\
\textbf{Term}: Definition

\subsubsection{Common considerations}
\begin{itemize}
    \item Consideration 1
    \item Consideration 2
\end{itemize}

\subsubsection{Examples of harms and implications}

% #RepresentationalHarm --> yellow
% #AllocativeHarm --> pink
% #QualityOfServiceHarm --> cyan
% #InterpersonalHarm --> lime
% #SocietalHarm --> orange

\begin{table}[H]
\caption{Example \#1: Example Name Here}
\centering
\begin{tabular}{|p{2cm}|p{13cm}|} % Fixed widths for the columns
\hline
\textbf{Harm Type(s)} &
  \textit{\textbf{\begin{tabular}[c]{@{}l@{}} \colorbox{lime}{\#HarmType} \\ → Sub-Harm-Type \end{tabular}}} \\ \hline
\textbf{Case Study} &
  Add Case Study Here. \\ \hline
\textbf{Harms \& \newline Implications} &
  And Harms and Implications Here. \\ \hline
\end{tabular}
\end{table}


\subsubsection{Mitigation Strategies}
Introduction to Mitigation Strategies here if there is one.


\underline{\textbf{Mitigation Strategy Header}}\\
Additional Info Here if there is any
\begin{itemize}
    \item Action item 1
    \item Action item 2
\end{itemize}
